ECI: a Customizable Cache Coherency Stack for Hybrid FPGA-CPU Architectures

Unlike other accelerators, FPGAs are capable of supporting cache coherency, thereby turning them into a more powerful architectural option than just a peripheral accelerator. However, most existing deployments of FPGAs are either non-cache coherent or support only an asymmetric design where cache coherency is controlled from the CPU. Taking advantage of a recently released two socket CPU-FPGA architecture, in this paper we describe ECI, a flexible implementation of cache coherency on the FPGA capable of supporting both symmetric and asymmetric protocols. ECI is open and customizable, given applications the opportunity to fully interact with the cache coherency protocol, thereby opening up many interesting system design and research opportunities not available in existing designs. Through extensive microbenchmarks we show that ECI exhibits highly competitive performance and discuss in detail one use-case illustrating the benefits of having an open cache coherency stack on the FPGA.

==> abstract.tex <==
\begin{abstract}
Modern, closely-coupled accelerators used in heterogeneous computer 
systems (GPUs, ASICs, FPGAs, etc) are often more powerful than the connected
CPUs. As a result,
 we must reconsider how they interact with the CPU, raising
many issues such as unified 
memory models between CPU and accelerators or cache coherency. 
In this paper we focus on cache coherency and present \eci, an open
system interconnect which directly interoperates with the full,
native, inter-socket coherence protocol on a modern CPU. Unlike
proposals presenting a high-level coherent interface to
accelerators, \eci~ can expose individual coherence messages, leading
to this insight: the directory functionality for tracking cache lines
can be usefully factored out of data movement and caching \emph{per
  se}. This ``deconstruction” of coherence allows even an existing
protocol to be subsetted by a specialized accelerator for efficiency,
or used in ways not possible with the complete protocol.
We have implemented \eci~ on the FPGA of a server-class heterogeneous 
computer system, and we discuss the challenges in talking
 directly to an existing CPU and cache.  We show through extensive microbenchmarks that
 \eci~ exhibits highly competitive performance and discuss in detail a
 number of use-cases exploiting the benefits of this  
broader perspective of what a deconstructed and open cache coherence 
protocol can do.
\end{abstract}

